Semantic HELM: A Human-Readable Memory for Reinforcement Learning

Reinforcement learning agents deployed in the real world often have to cope with partially observable environments. Therefore, most agents employ memory mechanisms to approximate the state of the environment. Recently, there have been impressive success stories in mastering partially observable environments, mostly in the realm of computer games like Dota 2, StarCraft II, or MineCraft. However, existing methods lack interpretability in the sense that it is not comprehensible for humans what the agent stores in its memory. In this regard, we propose a novel memory mechanism that represents past events in human language. Our method uses CLIP to associate visual inputs with language tokens. Then we feed these tokens to a pretrained language model that serves the agent as memory and provides it with a coherent and human-readable representation of the past. We train our memory mechanism on a set of partially observable environments and find that it excels on tasks that require a memory component, while mostly attaining performance on-par with strong baselines on tasks that do not. On a challenging continuous recognition task, where memorizing the past is crucial, our memory mechanism converges two orders of magnitude faster than prior methods. Since our memory mechanism is human-readable, we can peek at an agent's memory and check whether crucial pieces of information have been stored. This significantly enhances troubleshooting and paves the way toward more interpretable agents.

==> tables/avalon_hns_50m.tex <==
\begin{table}[t]
\begin{center}
\begin{tabular}{l c c c c c}
\toprule
Task & PPO & Dreamerv2 & HELM & HELMv2 & SHELM \\
\midrule
eat & 0.889 $\pm$ 0.074 & 0.664 $\pm$ 0.065 & 0.925 $\pm$ 0.075 & 0.690 $\pm$ 0.064 & 0.833 $\pm$ 0.075 \\
move & 0.421 $\pm$ 0.078 & 0.364 $\pm$ 0.071 & 0.373 $\pm$ 0.076 & 0.266 $\pm$ 0.058 & 0.288 $\pm$ 0.059 \\
jump & 0.288 $\pm$ 0.065 & 0.234 $\pm$ 0.058 & 0.309 $\pm$ 0.059 & 0.196 $\pm$ 0.048 & 0.233 $\pm$ 0.056 \\
climb & 0.257 $\pm$ 0.052 & 0.227 $\pm$ 0.051 & 0.207 $\pm$ 0.049 & 0.130 $\pm$ 0.042 & 0.046 $\pm$ 0.176 \\
descend & 0.205 $\pm$ 0.056 & 0.290 $\pm$ 0.058 & 0.226 $\pm$ 0.051 & 0.155 $\pm$ 0.041 & 0.206 $\pm$ 0.044 \\
scramble & 0.496 $\pm$ 0.068 & 0.422 $\pm$ 0.058 & 0.352 $\pm$ 0.063 & 0.238 $\pm$ 0.052 & 0.311 $\pm$ 0.058 \\
stack & 0.083 $\pm$ 0.036 & 0.126 $\pm$ 0.043 & 0.079 $\pm$ 0.032 & 0.077 $\pm$ 0.032 & 0.096 $\pm$ 0.038 \\
bridge & 0.051 $\pm$ 0.028 & 0.121 $\pm$ 0.045 & 0.021 $\pm$ 0.018 & 0.027 $\pm$ 0.019 & 0.045 $\pm$ 0.025 \\
push & 0.138 $\pm$ 0.048 & 0.160 $\pm$ 0.043 & 0.118 $\pm$ 0.043 & 0.068 $\pm$ 0.028 & 0.125 $\pm$ 0.041 \\
throw & 0.000 $\pm$ 0.000 & 0.000 $\pm$ 0.000 & 0.000 $\pm$ 0.000 & 0.000 $\pm$ 0.000 & 0.000 $\pm$ 0.000  \\
hunt & 0.032 $\pm$ 0.024 & 0.063 $\pm$ 0.028 & 0.062 $\pm$ 0.030 & 0.058 $\pm$ 0.029 & 0.052 $\pm$ 0.026   \\
fight & 0.292 $\pm$ 0.071 & 0.336 $\pm$ 0.076 & 0.219 $\pm$ 0.058 & 0.244 $\pm$ 0.059 &0.193 $\pm$ 0.054   \\
avoid & 0.383 $\pm$ 0.091 & 0.515 $\pm$ 0.118 & 0.320 $\pm$ 0.062 & 0.236 $\pm$ 0.082 & 0.187 $\pm$ 0.044 \\
explore & 0.222 $\pm$ 0.059 & 0.190 $\pm$ 0.048 & 0.254 $\pm$ 0.061 & 0.171 $\pm$ 0.046 & 0.219 $\pm$ 0.050 \\
open & 0.053 $\pm$ 0.026 & 0.126 $\pm$ 0.041 & 0.096 $\pm$ 0.034 & 0.113 $\pm$ 0.039 & 0.117 $\pm$ 0.040  \\
carry & 0.122 $\pm$ 0.049 & 0.066 $\pm$ 0.028 & 0.085 $\pm$ 0.037 & 0.076 $\pm$ 0.032 & 0.095 $\pm$ 0.042  \\
\midrule
navigate & 0.009 $\pm$ 0.010 & 0.000 $\pm$ 0.000 & 0.003 $\pm$ 0.005 & 0.000 $\pm$ 0.000 & 0.009 $\pm$ 0.011\\
find & 0.000 $\pm$ 0.000 & 0.000 $\pm$ 0.000 & 0.007 $\pm$ 0.009 & 0.000 $\pm$ 0.000 & 0.000 $\pm$ 0.000\\
survive & 0.045 $\pm$ 0.015 & 0.044 $\pm$ 0.014 & 0.056 $\pm$ 0.016 & 0.046 $\pm$ 0.015 & 0.053 $\pm$ 0.016\\
gather & 0.020 $\pm$ 0.010 & 0.021 $\pm$ 0.012 & 0.012 $\pm$ 0.007 & 0.007 $\pm$ 0.005 & 0.009 $\pm$ 0.004\\
\midrule
overall & \textbf{0.200 $\pm$ 0.013} & 0.199 $\pm$ 0.012 & 0.186 $\pm$ 0.012 & 0.140 $\pm$ 0.011 &  0.162 $\pm$ 0.010\\
\bottomrule
\end{tabular}
\end{center}
\caption{Mean human normalized score for for all Avalon tasks for PPO, HELMv2, and SHELM after 50M interaction steps. We show mean and standard deviations.}
\label{tab:avalon_hns_50m}
\end{table}

==> tables/avalon_main.tex <==
\begin{table}[t]
\caption{Average success rates over all tasks in Avalon for PPO, HELMv2, and \ourmethod.}
\label{tab:avalon_main}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{l c}
 PPO & 0.165 $\pm$ 0.014  \\\midrule
 HELMv2 & 0.167 $\pm$ 0.025 \\\midrule
 \ourmethod & \textbf{0.176} $\pm$ \textbf{0.031}\\
 \bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}

==> tables/avalon_task_success_rates.tex <==
\begin{table}[t]
\caption{Average success rates for for all Avalon tasks for PPO, HELMv2, and \ourmethod.}
\label{tab:avalon_task_succ_rates}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{l c c c}
\toprule
Task & PPO & HELMv2 & SHELM  \\
\midrule
eat & 0.708 $\pm$ 0.067 & 0.627 $\pm$ 0.109 & 0.633 $\pm$ 0.062\\
move & 0.311 $\pm$ 0.062 & 0.307 $\pm$ 0.034 & 0.313 $\pm$ 0.053\\
jump & 0.220 $\pm$ 0.050 & 0.267 $\pm$ 0.041 & 0.307 $\pm$ 0.025\\
climb & 0.193 $\pm$ 0.043 & 0.193 $\pm$ 0.041 & 0.253 $\pm$ 0.050\\
descend & 0.179 $\pm$ 0.043 & 0.49 $\pm$ 0.1 & 0.542 $\pm$ 0.11\\
scramble & 0.306 $\pm$ 0.054 & 0.28 $\pm$ 0.086 & 0.327 $\pm$ 0.100\\
stack & 0.091 $\pm$ 0.036 & 0.267 $\pm$ 0.057 & 0.233 $\pm$ 0.057\\
bridge & 0.049 $\pm$ 0.027 & 0.000 $\pm$ 0.000 & 0.007 $\pm$ 0.009\\
push & 0.113 $\pm$ 0.039 & 0.127 $\pm$ 0.053 & 0.073 $\pm$ 0.077\\
throw & 0.000 $\pm$ 0.000 & 0.007 $\pm$ 0.009 & 0.007 $\pm$ 0.009\\
hunt & 0.043 $\pm$ 0.024 & 0.04 $\pm$ 0.016 & 0.073 $\pm$ 0.009 \\
fight & 0.199 $\pm$ 0.052 & 0.085 $\pm$ 0.009 & 0.111 $\pm$ 0.009 \\
avoid & 0.493 $\pm$ 0.170 & 0.204 $\pm$ 0.091 & 0.179 $\pm$ 0.141\\
explore & 0.193 $\pm$ 0.047 & 0.16 $\pm$ 0.016 & 0.160 $\pm$ 0.028\\
open & 0.055 $\pm$ 0.024 & 0.233 $\pm$ 0.161 & 0.253 $\pm$ 0.025\\
carry & 0.073 $\pm$ 0.031 & 0.096 $\pm$ 0.031 & 0.090 $\pm$ 0.040\\
\midrule
navigate & 0.000 $\pm$ 0.000 & 0.000 $\pm$ 0.000 & 0.000 $\pm$ 0.000\\
find & 0.002 $\pm$ 0.003 & 0.000 $\pm$ 0.000 & 0.000 $\pm$ 0.000\\
gather & 0.021 $\pm$ 0.010 & 0.000 $\pm$ 0.000 & 0.000 $\pm$ 0.000\\
survive & 0.043 $\pm$ 0.013 & 0.000 $\pm$ 0.000 & 0.000 $\pm$ 0.000\\
\midrule
overall & 0.165 $\pm$ 0.014 & 0.167 $\pm$ 0.025 & \textbf{0.176} $\pm$ \textbf{0.031} \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}
